How Hard is Asynchronous Weight Reassignment? (Extended Version)

The performance of distributed storage systems deployed on wide-area networks can be improved using weighted (majority) quorum systems instead of their regular variants due to the heterogeneous performance of the nodes. A significant limitation of weighted majority quorum systems lies in their dependence on static weights, which are inappropriate for systems subject to the dynamic nature of networked environments. To overcome this limitation, such quorum systems require mechanisms for reassigning weights over time according to the performance variations. We study the problem of node weight reassignment in asynchronous systems with a static set of servers and static fault threshold. We prove that solving such a problem is as hard as solving consensus, i.e., it cannot be implemented in asynchronous failure-prone distributed systems. This result is somewhat counter-intuitive, given the recent results showing that two related problems -- replica set reconfiguration and asset transfer -- can be solved in asynchronous systems. Inspired by these problems, we present two versions of the problem that contain restrictions on the weights of servers and the way they are reassigned. We propose a protocol to implement one of the restricted problems in asynchronous systems. As a case study, we construct a dynamic-weighted atomic storage based on such a protocol. We also discuss the relationship between weight reassignment and asset transfer problems and compare our dynamic-weighted atomic storage with reconfigurable atomic storage.

==> tables/atomic-storage.tex <==
% \begin{table}[hbt!]
%     \centering
%     \caption{Our dynamic-weighted atomic storage v.s. reconfigurable atomic storage.}
%     \label{tbl:comparing-reconfigurable-objects}
%     \begin{tabular}{|l|c|c|}
%       \hline
%              \parbox[l]{0.92in}{} 
%            & \parbox[c]{0.9in}{Dynamic-weighted atomic storage (this paper)} 
%            & \parbox[c]{1.1in}{Reconfigurable atomic storage \cite{dynAtomicStorageWithoutCons, effModConsensus-freeFST, jehl2017case, smartMerge, spiegelman2017dynamic}} \\
%       \hline
%              \parbox[l]{0.92in}{Can be implemented in asynchronous failure-prone distributed systems?} 
%            & \parbox[c]{0.9in}{Yes} 
%            & \parbox[c]{1.1in}{Yes} \\
%       \hline
%              \parbox[l]{0.92in}{The fault-threshold} 
%            & \parbox[c]{0.9in}{Static and weighted} 
%            & \parbox[c]{1.1in}{Dynamic} \\
%       \hline
%              \parbox[l]{0.92in}{The system’s size} 
%            & \parbox[c]{0.9in}{Static} 
%            & \parbox[c]{1.1in}{Dynamic} \\
%       \hline
%              \parbox[l]{0.92in}{Availability condition} 
%            & \parbox[c]{0.9in}{The system remains available as long as the number of failures does not exceed the fault threshold.} 
%            & \parbox[c]{1.1in}{The system remains available as long as any pending configuration has a majority of servers that did not crash and were not proposed for removal.} \\
%       \hline
%     \end{tabular}
% \end{table}

% \begin{table}[hbt!]
%     \centering
%     \caption{Our dynamic-weighted atomic storage v.s. reconfigurable atomic storage.}
%     \label{tbl:comparing-reconfigurable-objects}
%     \begin{tabular}{|m{0.92in}|m{0.9in}|m{1.1in}|}
%       \hline
%              & Dynamic-weighted atomic storage (this paper) 
%            & Reconfigurable atomic storage \cite{dynAtomicStorageWithoutCons, effModConsensus-freeFST, jehl2017case, smartMerge, spiegelman2017dynamic} \\
%       \hline
%              Can be implemented in asynchronous failure-prone systems? 
%            & Yes 
%            & Yes \\
%       \hline
%              Fault-threshold 
%            & Static and weighted 
%            & Dynamic \\
%       \hline
%              System’s size 
%            & Static 
%            & Dynamic \\
%       \hline
%              Availability condition 
%            & The system remains available as long as the number of failures does not exceed the fault threshold. 
%            & The system remains available as long as any pending configuration has a majority of servers that did not crash and were not proposed for removal. \\
%       \hline
%     \end{tabular}
% \end{table}

\begin{table}[t!]
    \centering
    \caption{Our dynamic-weighted atomic storage v.s. reconfigurable atomic storage.}
    \label{tbl:comparing-reconfigurable-objects}
    \begin{tabular}{|>{\raggedright\arraybackslash}m{1.02in}|>{\raggedright\arraybackslash}m{0.85in}|>{\raggedright\arraybackslash}m{1.07in}|}
        \hline
        \multicolumn{1}{|>{\raggedright\arraybackslash}m{1.02in}|}{\vspace{0pt}}
        & \multicolumn{1}{>{\raggedright\arraybackslash}m{0.85in}|}{\vspace{1pt}Dynamic-weighted atomic storage (this paper)}
        & \multicolumn{1}{>{\raggedright\arraybackslash}m{1.07in}|}{\vspace{-8pt}Reconfigurable atomic storage \cite{dynAtomicStorageWithoutCons, effModConsensus-freeFST, jehl2017case, smartMerge, spiegelman2017dynamic}} \\
        \hline
        Can be implemented in asynchronous failure-prone systems? & Yes & Yes \\
        \hline
        Fault-threshold & Static and weighted & Dynamic \\
        \hline
        System’s size & Static & Dynamic \\
        \hline
        Availability condition & \multicolumn{1}{>{\raggedright\arraybackslash}m{0.85in}|}{\vspace{-18pt}The system remains available as long as the number of failures does not exceed the fault threshold.} & The system remains available as long as any pending configuration has a majority of servers that did not crash and were not proposed for removal. \\
        \hline
    \end{tabular}
\end{table}


% \begin{table}[hbt!]
%     \centering
%     \caption{Our dynamic-weighted atomic storage v.s. reconfigurable atomic storage.}
%     \label{tbl:comparing-reconfigurable-objects}
%     % \hspace{0.1em}
%     \begin{tabular}{m{0.92in}|m{0.9in}|m{1.1in}|}
%       \cline{2-3}
%            & \centering Dynamic-weighted atomic storage (this paper) 
%            & \centering\arraybackslash Reconfigurable atomic storage \cite{dynAtomicStorageWithoutCons, effModConsensus-freeFST, jehl2017case, smartMerge, spiegelman2017dynamic}
%     \end{tabular}
    
%     \begin{tabular}{|m{0.92in}|m{0.9in}|m{1.1in}|}
%       \hline
%            Can be implemented in asynchronous failure-prone distributed systems? 
%            & \centering Yes 
%            & \centering\arraybackslash Yes \\
%       \hline
%            The fault-threshold 
%            & \centering Static and weighted 
%            & \centering\arraybackslash Dynamic \\
%       \hline
%            The system’s size 
%            & \centering Static 
%            & \centering\arraybackslash Dynamic \\
%       \hline
%            Availability condition 
%            & \centering The system remains available as long as the number of failures does not exceed the fault threshold. 
%            & \centering\arraybackslash The system remains available as long as any pending configuration has a majority of servers that did not crash and were not proposed for removal. \\
%       \hline
%     \end{tabular}
% \end{table}


==> tables/pairwise-vs-asset-transfer.tex <==
\begin{table*}[hbt!]
    \centering
    \caption{Relation with the asset transfer problem}
    \label{tbl:pwr-vs-1-at}
    \begin{tabular}{|l|c|c|c|c|}
      \hline
             \parbox[l]{1.1in}{} 
           & \parbox[c]{1.3in}{Pairwise weight reassignment (this paper)} 
           & \parbox[c]{1.3in}{Restricted pairwise weight reassignment (this paper)} 
           & \parbox[c]{1.3in}{$k$-asset transfer} 
           & \parbox[c]{1.3in}{$1$-asset transfer} \\
      \hline
             \parbox[l]{1.1in}{Consensus number} 
           & \parbox[c]{1.3in}{at least $n-f$} 
           & \parbox[c]{1.3in}{1} 
           & \parbox[c]{1.3in}{$k$} 
           & \parbox[c]{1.3in}{1} \\
      \hline
             \parbox[l]{1.1in}{The Fault-threshold} 
           & \parbox[c]{1.3in}{Static and weighted} 
           & \parbox[c]{1.3in}{Static and weighted} 
           & \parbox[c]{1.3in}{Static and unweighted} 
           & \parbox[c]{1.3in}{Static and unweighted} \\
      \hline
             \parbox[l]{1.1in}{The system’s size} 
           & \parbox[c]{1.3in}{Static} 
           & \parbox[c]{1.3in}{Static} 
           & \parbox[c]{1.3in}{Static} 
           & \parbox[c]{1.3in}{Static} \\
      \hline
             \parbox[l]{1.1in}{The relationship between the quorum formation and weights/assets} 
           & \parbox[c]{1.3in}{The quorum formation depends on weights} 
           & \parbox[c]{1.3in}{The quorum formation depends on weights} 
           & \parbox[c]{1.3in}{The quorum formation is independent of assets} 
           & \parbox[c]{1.3in}{The quorum formation is independent of assets} \\
      \hline
             \parbox[l]{1.1in}{Is there any condition related to the distribution of weights/assets?} 
           & \parbox[c]{1.3in}{Yes (the total of the $f$ greatest weights should be less than half of the total weight)} 
           & \parbox[c]{1.3in}{Yes (the total of the $f$ greatest weights should be less than half of the total weight)} 
           & \parbox[c]{1.3in}{No} 
           & \parbox[c]{1.3in}{No} \\
      \hline
    \end{tabular}
\end{table*}
